POLYPATH: Supporting Multiple Tradeoffs for Interaction Latency

Modern mobile systems use a single input-to-display path to serve all applications. In meeting the visual goals of all applications, the path has a latency inadequate for many important interactions. To accommodate the different latency requirements and visual constraints by different interactions, we present POLYPATH, a system design in which application developers (and users) can choose from multiple path designs for their application at any time. Because a POLYPATH system asks for two or more path designs, we present a novel fast path design, called Presto. Presto reduces latency by judiciously allowing frame drops and tearing. We report an Android 5-based prototype of POLYPATH with two path designs: Android legacy and Presto. Using this prototype, we quantify the effectiveness, overhead, and user experience of POLYPATH, especially Presto, through both objective measurements and subjective user assessment. We show that Presto reduces the latency of legacy touchscreen drawing applications by almost half; and more importantly, this reduction is orthogonal to that of other popular approaches and is achieved without any user-noticeable negative visual effect. When combined with touch prediction, Presto is able to reduce the touch latency below 10 ms, a remarkable achievement without any hardware support.

==> async.tex <==
\subsection{Just-in-time Trigger}\label{sec:design_async}
The just-in-time trigger aims to remove synchronization at points \txtcircle{1} and \txtcircle{3}.
\jit triggers both event delivery (\txtcircle{1}) and buffer ownership transfer (\txtcircle{3}), asynchronously.
To determine the event delivery time, it predicts how much time an application will spend to process events and draw on a buffer.
Using the prediction, \async carefully triggers the event delivery so that it is late enough for an application to receive more recent events, but early enough not to miss the next screen update.
We discuss the prediction in detail in \S~\ref{sec:design_prediction}.
To decide the buffer ownership transfer time, \jit has to know how much time the buffer ownership transfer requires.
Focusing on a single main app highly simplifies the output subsystem's execution.
In our experiments with more than 6,000 execution time samples, 99.9\% of the samples are below 2.8 ms and all of them are below 3.5 ms.




\begin{figure*}[t]
	\begin{minipage}[t]{0.48\textwidth}
		\centering
		\includegraphics[width=1\columnwidth]{figs/design_async.pdf}
		\caption{Latency from just-in-time trigger: 
			The input subsystem delivers more recent events by predicting the application's execution time.
			A wrong prediction, however, adds an extra $T_{sync}$ latency for the frame $F_{2:3}$.}
		\label{fig:design_async}
	\end{minipage}
	\hfill
	\begin{minipage}[t]{0.48\textwidth}
		\centering
		\includegraphics[width=1\columnwidth]{figs/design_async_bypass.pdf}
		\caption{Latency from just-in-time frame delivery: 
			The recovery procedure drops the frame $F_{2:3}$ with a wrong prediction and avoids propagating delays.}
		\label{fig:design_async_bypass}
	\end{minipage}
	\vspace{-3mm}
\end{figure*}

Figure~\ref{fig:design_async} illustrates how the just-in-time trigger works.
When $E_0$ happens, the input subsystem has the two predicted execution times for the application and the output subsystem.
The next event $E_1$ can be processed before the next \vsync, thus the input subsystem waits for the event.
On the contrary, the input subsystem does not wait for $E_2$ because the event cannot be processed before the next \vsync.
As a result, the waiting reduces the latency for $E_1$ because the application processes it before $V_1$ and the output subsystem successfully transfers $F_{0:1}$'s ownership to the display subsystem by $V_1$.
It is worth noting that the waiting does not increase the latency for $E_0$ because both \async and a legacy system finish processing the event before the $V_1$.

$ and $T_{output}$. Yet your text below suggests JIT reduces $T_{app}$ and $T_{out}$. Confusing}
The latency model with just-in-time trigger is:
\begin{equation}\label{eq:jitt}
\bar{T} = \bar{T}_{input} + \boldsymbol{T'}_{\boldsymbol{app}} + \boldsymbol{T'}_{\boldsymbol{out}} + \bar{T}_{disp} 
\end{equation}
Compared to the base model, Equation \eqref{eq:base}, $T_{app}$ and $T_{out}$ is changed to $T'_{app}$ and $T'_{out}$, respectively.
$T'_{app}$ is introduced by the first trigger at \txtcircle{1} and it represents an application's predicted execution time to process the event and render a frame.
$T'_{out}$ is introduced by the second trigger at \txtcircle{3}, and it is 3.5 ms.
Hence, the just-in-time trigger reduces 
\begin{equation}\label{eq:jitt_reduce}
22.4_{(ms)} - T'_{app} (= T_{app} + T_{out} - T'_{app} - T'_{out})
\end{equation}
from the equation~\eqref{eq:base}.


Underprediction of the application execution time, however, may happen and introduce delay to equation \eqref{eq:jitt}.
\jit provides a recovery mechanism described in \S~\ref{sec:design_bypass}.





\input{prediction}
\input{bypass}

